Parallel Integer Sort: Theory and Practice

Integer sorting is a fundamental problem in computer science. This paper studies parallel integer sort both in theory and in practice. In theory, we show tighter bounds for a class of existing practical integer sort algorithms, which provides a solid theoretical foundation for their widespread usage in practice and strong performance. In practice, we design a new integer sorting algorithm, \textsf{DovetailSort}, that is theoretically-efficient and has good practical performance. In particular, \textsf{DovetailSort} overcomes a common challenge in existing parallel integer sorting algorithms, which is the difficulty of detecting and taking advantage of duplicate keys. The key insight in \textsf{DovetailSort} is to combine algorithmic ideas from both integer- and comparison-sorting algorithms. In our experiments, \textsf{DovetailSort} achieves competitive or better performance than existing state-of-the-art parallel integer and comparison sorting algorithms on various synthetic and real-world datasets.

==> exp-merge.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.8\columnwidth]{output/32bit-merge.pdf}\\\vspace{-.8em}(d)
  \caption{
  \textbf{Analysis for the performance of dovetail merging (lower is better).}
  Discussions are in \cref{sec:exp-study}.
  }\label{fig:exp:merge}
\end{figure}




==> figures/merge_text.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=2\columnwidth]{figures/merge.pdf}
    \caption{\small \textbf{Our merge subroutine.}
    }\label{fig:merge}
  \end{figure*} 

==> intro-conflict.tex <==
\section{Introduction}\label{sec:intro}

Sorting is one of the most widely-used primitives in algorithm design, and has been extensively studied in computer science.
%
For many if not most cases in practice, the keys of the records to be sorted are fixed-length integers.
%
Algorithms that take advantage of integer input keys are referred to \emp{integer sorting algorithms}.
%
An integer sorting algorithm takes as input $n$ records with keys in the range 0 to $r-1$, and must output the records with keys in a non-decreasing order (formally defined in \cref{sec:prelim}).
%
Despite decades of effort on designing improved integer sorting
algorithms, however, obtaining integer sorting algorithms that are
{\em efficient both in theory and in practice} has remained elusive.
%there have been unanswered challenges on parallel integer sort, \emp{both in theory and in practice}.
%In this paper, we study the theory and practice of parallel integer sorts.

\myparagraph{Theoretical challenges.}
As a special instance of sorting, integer sorting algorithms \emp{can}
outperform comparison-based sorting algorithms by taking advantage of
the bitwise encoding of the keys.
%
%since they can directly work on the bits of the keys.
%Such a claim is verified in our experiments (e.g., \cref{fig:heatmap}), on the state-of-the-art parallel integer sorting algorithms~\cite{blelloch2020parlaylib,obeya2019theoretically,axtmann2022engineering} and comparison sorting algorithms~\cite{blelloch2020parlaylib,axtmann2022engineering}.
%
Indeed in many existing studies~\cite{obeya2019theoretically,axtmann2022engineering} and our own experiments (see \cref{fig:heatmap}), integer sorts outperform comparison sorts in many cases.  %on general inputs with all distinct keys.
%
This is also why many real-world applications that utilize integer keys (e.g., graph transposing in some graph libraries~\cite{}) choose to use integer sorts other than general comparison sorts.
%
While the fact that integer sorts can outperform comparison sorts is not surprising, we observe a \emph{significant gap} in connecting the high performance with theory.
%
Although there have been algorithms with good bounds~\cite{bhatt1991improved,albers1997improved,andersson1998sorting}, these algorithms are quite complicated, and we are unaware of any implementations of them.
%
On the other hand, for all the existing integer sort implementations with high performance~\cite{blelloch2020parlaylib,obeya2019theoretically,axtmann2022engineering}, we are unaware of ``meaningful'' analysis for them.
%
In particular, the best known bounds for these algorithms, as discussed in~\cite{obeya2019theoretically}, are $O(n\log r)$ work (number of operations) and $\polylog(rn)$ span (longest dependence chain).
%
However, the bounds are no better than comparison sort ($O(n\log n)$ work and $O(\log n)$ span~\cite{blelloch2020optimal,goodrich2023optimal}\footnote{Or $\polylog(n)$ span for practical implementations~\cite{blelloch2010low,blelloch2020parlaylib}.}) when $r=\Omega(n)$\footnote{When $r=o(n)$, one should directly use parallel counting sort with $O(n)$ work and $O(\log n)$ span~\cite{RR89,blelloch2020optimal} (see \cref{sec:counting}).}.
%
This conclusion obviously contradicts with the experimental results, for instance those in \cref{fig:heatmap}.

\hide{
\myparagraph{Practical challenges.}
Meanwhile, as a special type of sorting, integer sorting algorithms \emp{should} outperform comparison sorting algorithms by taking advantage of the integer bits information.
In fact, one should always consider comparison sort as a baseline for sorting integers as integers are comparable.
Unfortunately, even on standard 32-bit integers, SOTA integer sorting algorithms still face significant challenges to outperform comparison sorts.
%One such difficulty is that parallel integer sorts naturally \emph{suffer significant performance degradation for inputs with many duplicate keys}, which are realistic and %frequently occur in practice.
One such challenge comes from the inherent difficulty to deal with \emph{duplicate keys}.
In particular, existing parallel integer sorting algorithms follow the most-significant digit (MSD) framework that uses 8--12 highest bits to first partition all keys into buckets, and recurse on the next several bits within each bucket in parallel.
%Thus, the case where the keys are uniform in a large key range is probably the most advantageous---due to the uniform distribution, the buckets (and thus the parallel tasks) are roughly load-balanced.
Heavy duplicate keys may make the subproblems unbalanced.
On the other hand, most comparison sorting algorithms naturally can identify and thus benefit from heavy duplicates in the input, and achieve much better performance than the general case (see xx).
For example, sample sort can skip a recursive subproblem once two samples have the same key, and quicksort can also separate keys equal to the pivot in partition, and avoid further processing them.
%However, duplications are hard to be utilized by integer sorts, since the subproblems are divided by the integer bits: as long as there is a
Interestingly, such a case does not apply to integer sorts.
To understand this, one can consider a simple input with $n-1$ keys $x$ and one key $x+1$.
In most comparison sorts, the heavy duplicates of $x$ simplify the problem and the complexity would degenerate to $O(n)$.
However, for parallel integer sorts, all computations until the base case level make no progress to distinguish $x$ and $x+1$,
causing much redundant work. In \cref{tab:xx}, we can see that on distributions with heavy duplicates, existing integer sorts can be much slower than
%In particular, existing parallel integer sorting algorithms follow the general framework that uses 8--12 most-significant bits in the keys to first partition all keys into buckets, and recurse on the next several bits within each bucket in parallel.
%Thus, the case where the keys are mostly distinct is probably the simplest and most advantageous---due to the uniform distribution, the buckets (and thus the parallel tasks) are roughly load-balanced.
%so all records will be sorted after only a small number of rounds.
%For comparison sorts, such a case is also the most general
%As an example, in \cref{fig:heatmap}, the input \texttt{uniform-}$10^9$ (each key is uniformly drawn from 0 to $10^9$),
%is almost the fastest case for an existing integer sort \plis{}~\cite{}, and one of the slowest cases for the comparison sorts \plss{}~\cite{} and \ipso{}~\cite{}.
%The overall trends are similar for other integer sorting algorithms since they share similarities at a high level.
}

\myparagraph{Practical challenges.}
\emph{As a specialized sorting algorithms, integer sorting algorithms \textbf{should} outperform comparison sorting algorithms by taking advantage of the integer encoding of keys.}
%
In fact, since integers are comparable, one should always consider comparison sort as a baseline for sorting integers.
%
Unfortunately, state-of-the-art (SOTA) parallel integer sorting algorithms do not consistently outperform the best parallel comparison-based sorting algorithms.
%
%One such difficulty is that parallel integer sorts naturally \emph{suffer significant performance degradation for inputs with many duplicate keys}, which are realistic and %frequently occur in practice.
One reason is due to the inherent difficulty of dealing with \emph{duplicate keys} in integer sorts.
%
In principle, duplicate keys are beneficial for sorting algorithms. 
%For most comparison sorting algorithms it is naturally easy to identify and thus benefit from heavy duplicates, and achieve much better performance than the general case (see xx).
%as the most widely used parallel comparison sorting algorithm, 
For example, {\em samplesort} can skip a recursive subproblem between two samples if both samples have the same key; similarly, quicksort can separate keys equal to the pivot in partition to avoid further processing them.
%
Interestingly, we are not aware of any existing integer sorts that utilize similar ideas that can benefit from duplicate keys.
%
In particular, existing parallel integer sorting algorithms follow the
{\em most-significant digit (MSD)} framework that first partitions all
keys into buckets based on the 8--12 highest bits, and recurses on the
next several bits within each bucket.
%
Equivalent keys are not detected until the last level of the recursion
(the base cases). 
%
Consider the extreme case where all or almost all records have the same key.
%
Samplesort or quicksort implementations easily achieve $O(n)$ work on
this instance.
%
However, to the best our knowledge, no existing parallel integer sorting 
implementation can handle this instance in a non-trivial manner. 
%
\cref{tab:xx} shows that on distributions with heavy duplicates (e.g., a uniform distribution with a small number of distinct keys), existing integer sorts can be slower than comparison sorts.\footnote{
We note that some techniques in existing integer sorting algorithms (e.g., \regions{}~\cite{obeya2019theoretically} and \ipsra{}~\cite{axtmann2022engineering}) have a side-effect to benefit from duplicates in some cases, at a cost of making the algorithms \emph{unstable}.  In this paper we want to overcome this issue without sacrificing stability.
}

%(although this is not their main goal). However, the corresponding techniques (usually those to make them in-place) unfortunately made the algorithms \emph{unstable}.}.
%In particular, existing parallel integer sorting algorithms follow the general framework that uses 8--12 most-significant bits in the keys to first partition all keys into buckets, and recurse on the next several bits within each bucket in parallel.
%Thus, the case where the keys are mostly distinct is probably the simplest and most advantageous---due to the uniform distribution, the buckets (and thus the parallel tasks) are roughly load-balanced.
%so all records will be sorted after only a small number of rounds.
%For comparison sorts, such a case is also the most general
%As an example, in \cref{fig:heatmap}, the input \texttt{uniform-}$10^9$ (each key is uniformly drawn from 0 to $10^9$),
%is almost the fastest case for an existing integer sort \plis{}~\cite{}, and one of the slowest cases for the comparison sorts \plss{}~\cite{} and \ipso{}~\cite{}.
%The overall trends are similar for other integer sorting algorithms since they share similarities at a high level.

\hide{
However, existing integer sorting algorithms become much slower for inputs with many duplicate keys.
In principle duplicate keys can be beneficial for sorting algorithms, since records with the same key are considered ties and do not need further sorting.
Unfortunately, existing integer sorting algorithms cannot take this advantage, and it is even worse that highly duplicate keys will cause imbalanced recursive subproblem sizes and more rounds to finish.
In contrast, comparison sorting algorithms such as PLSS~\cite{blelloch2020parlaylib} and IPS$^4$o~\cite{axtmann2022engineering}, which are variants of samplesort, take advantage of duplicate keys inherently by the sampling schemes in the algorithms.
When a duplicate key has many occurrences, it can get more than one sampled pivots that form its own bucket, and no further sorting is needed.
Given the ebb and flow, existing integer sorting can be slower than comparison sorting when the occurrences of duplicate keys are high (see \cref{fig:heatmap} and \cref{tab:overall}).
}

\myparagraph{Our contributions.} In this paper, we study parallel integer sort to overcome the aforementioned challenges both in theory and in practice.
In theory, \emph{we close the gap between theory and practice by proving that \textbf{a class of} parallel integer sorting algorithms, including our new algorithm that will be proposed in this paper, have $O(n\sqrt{\log r})$ work for an input of $n$ integers in range $0$ to $r-1$}. 
This is asymptotically better than comparison sorts for a large key range $r=o(n^{\sqrt{\log n}})$.
This explains why the existing integer sorts are indeed faster than comparison sorts in practice in many cases. 
We also show that we can achieve $\polylog(nr)$ span \whp{} for an unstable integer sort, and $\tilde{O}(2^{\sqrt{\log r}})$ span for a class of practical stable algorithms such as our new \oursort{} and the integer sort in ParlayLib~\cite{blelloch2020parlaylib}. Note that the term $2^{\sqrt{\log r}}$ in the span bound is subpolynomial. 
We also proved that new algorithm has $\Theta(n)$ work for some special input distributions with heavy duplicates. 
In addition to the new bounds, the theory developed in this paper (\cref{sec:theory}) 
also explains the choices of parameters in practice for many (if not all) parallel integer sorts. 
%We believe the intellectual merit of this analysis is novel and significant.
%We believe that our analysis gives the first non-trivial work bound on practical parallel integer sorts.
%
We believe that our theoretical contribution is important both for
analyzing our own algorithm and for understanding parallel integer
sort as a general problem.
%
%We believe that our contribution is important both for analyzing our own algorithm,
%as well as for closing the gap between theory and practice for the parallel integer sort problem.

In practice, \emph{we propose \oursortfull{} (\oursort{}), an parallel
integer sorting algorithm that is \textbf{efficient, stable, and
race-free}}.\laxman{race-free or determinacy-race-free?}
%
\oursort{} combines algorithmic ideas from both integer- and
comparison-sorting algorithms.
%
%The backbone of our algorithm is still based on integer sort since it can efficiently sort lightly duplicate keys (the ``light keys'').
%Our key innovation is to integrate a set of techniques into integer sorts, such that
%
The goal is to let the algorithm detect and take advantage of heavily
duplicated keys (the \emp{heavy keys}) by sampling and performing
comparisons, but preserve the low asymptotic work bound as in an
integer sorting algorithm by using the integer encodings of keys.
\laxman{changed integer bits information --> integer encodings or
bitwise encodings of keys in multiple places}
%
%remain %remain at a low cost when the number of heavy keys is small.
%Our key innovation is to integrate the ideas from comparison-based sort and semisorting algorithms into integer sorts, such that the algorithm can separate the \emp{heavy keys} (i.e., keys with heavy duplicates) from \emp{light keys} (i.e., the other keys),
%but remains at a low cost when the number of heavy keys is small.
%
The key idea is to 1) use sampling to identify and gather heavy keys
and separate them from the other keys (called \emp{light keys}) and
prevent them being passed into the recursive calls, 
%
and 2) exploit the bitwise encoding of the keys to split light keys
into subproblems and deal with them recursively.

Although the high-level idea of \emph{separating} heavy keys and light
keys is quite natural, an interesting challenge is that the all keys
need to be stored in increasing order in the output, and thus the
heavy and light keys have to be finally \emph{interleaved} with each
other.
%
Therefore, the heavy-light separation idea requires \emp{dovetailing}
the keys efficiently (in terms of work, depth, and cache-efficiency).
%
Our idea is to first carefully place the heavy keys close to their
final destinations at the initial stage. \laxman{initial stage is
unclear here}
%
After the light keys have been locally sorted from the recursive
calls, we employ a dedicated algorithm to combine them into the final
sorted order.
%
We present details of our algorithm in \cref{sec:oursort} and analysis
in \cref{sec:theory}.
%
%Despite the benefit of separating the heavy keys, we note that an additional
%This process employs comparisons on the keys, and
%Note that now the heavy and light keys are processed separately and must be combined in the final output.
\hide{
A na\"ive parallel merge will be very costly here, especially due to the recursive structure of integer sort.
Hence, such merging must be applied at every level, offsetting the benefit of distinguishing heavy keys from light keys (see \cref{sec:exp} for details).
In comparison, our techniques will carefully put heavy keys ``close to'' their final destinations, and deploy a sophisticated yet efficient in-place algorithm to shuffle them to the correct final destinations.
In most cases, the cost of merging is roughly proportional to the smaller number of heavy or light keys in this subproblem.
More interestingly, our algorithm remains \emph{stable} and \emph{race-free} (see definitions in \cref{sec:prelim}), which are key features for sorting algorithms and parallel algorithms, respectively. %\yan{Need to mention some theory, but we can only work on that when the algorithm part is almost done.}
}


\hide{
Integer sorting algorithms can outperform comparison sorting algorithms since they can directly work on the bits of the keys.
Such a claim is verified in our experiments (e.g., \cref{fig:heatmap}), on the state-of-the-art parallel integer sorting algorithms~\cite{blelloch2020parlaylib,obeya2019theoretically,axtmann2022engineering} and comparison sorting algorithms~\cite{blelloch2020parlaylib,axtmann2022engineering}.
 %on $10^9$ records with 32-bit key-value pairs on various distributions, among three state-of-the-art parallel integer sorting algorithms: ParlayLib Integer Sort (PLIS)~\cite{blelloch2020parlaylib}, RegionSort~\cite{obeya2019theoretically}, and IPS2Ra~\cite{axtmann2022engineering}, and two comparison sorting algorithms: ParlayLib SampleSort (PLSS)~\cite{blelloch2020parlaylib} and IPS4o~\cite{axtmann2022engineering}.

\myparagraph{Theoretical challenges and our contributions.}
We note a \emph{significant gap} between the theory and practice of parallel integer sort.
Theoretically, there have been algorithms with good bounds~\cite{bhatt1991improved,albers1997improved,andersson1998sorting} but they are impractically complicated.
On the practice side, we are unaware of ``meaningful'' analysis for existing algorithms~\cite{blelloch2020parlaylib,obeya2019theoretically,axtmann2022engineering}.
The best known bounds are $O(n\log r)$ work (number of operations) and $\polylog(rn)$ span (longest dependence chain)~\cite{obeya2019theoretically}.
However, the bounds are no better than comparison sort ($O(n\log n)$ work and $O(\log n)$ span~\cite{blelloch2020optimal,goodrich2023optimal}\footnote{Or $\polylog(n)$ span for practical implementations~\cite{blelloch2010low,blelloch2020parlaylib}.}) when $r=\Omega(n)$\footnote{When $r=o(n)$, one should directly use parallel counting sort with $O(n)$ work and $O(\log n)$ span~\cite{RR89,blelloch2020optimal}.}.
This conclusion obviously contradicts with the experimental results, for instance those in \cref{fig:heatmap}.

In this paper, we close this long-standing gap between the theory and practice by showing that the integer sorting algorithms, including PLIS and our new \oursort, use $O(n\sqrt{\log r})$ work.
This explains why they are faster than comparison sort in practice, and asymptotically incur fewer operations in the range of $r=o(n^{\sqrt{\log n}})$.
We also show that we can achieve $O(\sqrt{\log r}\log n)$ span \whp{} for unstable integer sort, and $O(\sqrt{\log r}2^{\sqrt{\log n}})$ span for the practical PLIS and our \oursort.
The theory developed in this paper (in \cref{sec:theory}) explains the efficiency of the parallel integer sorting algorithms (including our \oursort), the asymptotic trends, and the choice of parameter in practice.
We believe the intellectual merit of this analysis is novel and significant.
}

%, they generally outperform the state-of-the-art parallel comparison sorting algorithms such as ParlayLib SampleSort (PLSS)~\cite{blelloch2020parlaylib} and IPS4o~\cite{axtmann2022engineering}.
\hide{
\myparagraph{Practical challenges and our contributions.}
The main challenge we observed for existing integer sorting algorithms is that \emph{they suffer significant performance degradation for inputs with many duplicate keys}, which are realistic and frequently occur in practice.
Existing parallel integer sorting algorithms follow the overall framework that look at 8--12 most-significant bits of the keys, distribute the records to the associated buckets, and recurse.
Thus, the case where the keys are distributed {\em uniformly with few duplicates} are probably the simplest and most advantageous---due to the keys being uniformly distributed, the buckets are roughly balanced, so all records will be sorted after only a small number of rounds.
As an example, in \cref{fig:heatmap}, the uniform case, e.g., \texttt{uniform-}$10^9$ (each key is uniformly drawn from 0 to $10^9$), is almost the fastest case for PLIS, and one of the slowest cases for PLSS and IPS$^4$o.
The overall trends are similar for other integer sorting algorithms since they share similarities at a high level.

However, existing integer sorting algorithms become much slower for inputs with many duplicate keys.
In principle duplicate keys can be beneficial for sorting algorithms, since records with the same key are considered ties and do not need further sorting.
Unfortunately, existing integer sorting algorithms cannot take this advantage, and it is even worse that highly duplicate keys will cause imbalanced recursive subproblem sizes and more rounds to finish.
In contrast, comparison sorting algorithms such as PLSS~\cite{blelloch2020parlaylib} and IPS$^4$o~\cite{axtmann2022engineering}, which are variants of samplesort, take advantage of duplicate keys inherently by the sampling schemes in the algorithms.
When a duplicate key has many occurrences, it can get more than one sampled pivots that form its own bucket, and no further sorting is needed.
Given the ebb and flow, existing integer sorting can be slower than comparison sorting when the occurrences of duplicate keys are high (see \cref{fig:heatmap} and \cref{tab:overall}).


\yan{Since we now have the theory part, we may want to significantly cut this paragraph, but kind of leave some ``ideas'' on why it is not trivial.}
In this paper, we try to understand whether the deficit of parallel integer sort in handling duplicate keys is inherent or not. %, given that in real-world cases, the input instances usually contain duplicate keys.
%An ideal parallel integer sorting algorithm should get faster when duplicate keys occur, but unfortunately we are unaware of any existing solutions.
One idea is to combine the ideas in checking the bits in integer sort and sampling scheme in comparison sort, but this is highly non-trivial since the high-level approaches in the two types of algorithms are quite different.
For instance, if we simply adopt the sampling scheme, we can now handle heavily duplicate keys easily, but the boundaries between the subproblems are no longer based on the binary representations of the integers, losing the benefit of integer inputs.
}



\hide{
This paper shows a novel approach to combine the advantages of both approaches.
The backbone of our algorithm is still based on integer sort since it can efficiently sort lightly duplicate keys (the ``light keys'').
Our key innovation is a set of techniques that can detect and deal with the heavily duplicate keys (the ``heavy keys''), but remains at a low cost when the number of heavy keys is small.
Note that now the heavy and light keys are processed separately and must be combined in the final output.
A na\"ive parallel merge will be very costly here, especially due to the recursive structure of integer sort.
Hence, such merging must be applied at every level, offsetting the benefit of distinguishing heavy keys from light keys (see \cref{sec:exp} for details).
In comparison, our techniques will carefully put heavy keys ``close to'' their final destinations, and deploy a sophisticated yet efficient in-place algorithm to shuffle them to the correct final destinations.
In most cases, the cost of merging is roughly proportional to the smaller number of heavy or light keys in this subproblem.
More interestingly, our algorithm remains \emph{stable} and \emph{race-free} (see definitions in \cref{sec:prelim}), which are key features for sorting algorithms and parallel algorithms, respectively. %\yan{Need to mention some theory, but we can only work on that when the algorithm part is almost done.}
}

\input{heatmap-fig.tex}

%Due to the novel algorithmic improvements, we believe our algorithm is the first parallel integer sorting algorithm that can benefit from duplicate keys instead of being at a disadvantage.
Due to the new algorithmic improvements, our \oursort{} achieves
consistently strong performance on various synthetic and real-world
input instances.
%
We present a summary of result in \cref{fig:heatmap}. 
%
Compared to the fastest existing integer sort \plis{}, our algorithm
is competitive (8\% faster) for no or very light duplicate keys (i.e.,
uniform-$10^9$), and can be up to 2.5$\times$ faster depending on the
amount of duplication, with a geometric mean of 27\% speedup.
%
The advantage of \oursort{} is larger (66\% faster) when keys are
64-bit integers---in this case \plis{} is no faster than
comparison-based samplesort due to a larger key range, while
\oursort{} is still faster. \laxman{faster than both? just PLIS? Are
results in \cref{fig:heatmap} for 64-bit keys?}
%
We also evaluate our algorithms into several applications with
real-world input data.
%
Our sorting algorithm is almost always the fastest, except for losing
to a comparison sort \ipso{} for a few cases, but is still the best
among all baselines in the overall (geometric mean) running time.
\laxman{It would be nice to say something like ``even for the
highly-optimized case of sequential sorting, there is no {\em best}
sorting algorithm; there are better and worse algorithms depending on
the use-case, and the goal is to design algorithms that are always
close-to-best in any use-case.''}
%
%---a comparison sort is probably more suitable for these cases---
%Considering the importance of sorting, we believe our algorithm is potentially useful to accelerate a wide range of applications.
%
We plan to make our code publicly available.\laxman{incorporate our
work in ParlayLib so it can be easily used?}
%
%Considering the importance of sorting and the amount of existing work, we believe our algorithm is an interesting alternative solution that one can always try to plug in their algorithms if possible, and expect a competitive or improved performance.

\hide{
\myparagraph{Our contributions on the theory side.}
Our paper also provides strong results on the theoretical side for parallel integer sort.
Despite some probably impractical theoretical work~\cite{}, the best known bounds for the practical integer sorting algorithms are $O(n\log r)$ work (number of operations) and $\polylog(rn)$ span (longest dependence chain)~\cite{obeya2019theoretically}.
It is well-known that comparison sort has $O(n\log n)$ work and $O(\log n)$ span~\cite{blelloch2020optimal,goodrich2023optimal} (or $\polylog(n)$ span for practical implementations~\cite{blelloch2010low}).
When comparing the bounds, integer sort is only advantageous when $r=o(n)$, but in this case, one should directly use parallel counting sort with $O(n)$ work and $O(\log n)$ span~\cite{RR89,blelloch2020optimal}.
When $r=\Omega(n)$, the theory indicates that comparison sort is always better, but this conclusion obviously contradicts with the experimental results, for instance those in \cref{fig:heatmap}.

In this paper, we close this long-standing gap between the theory and practice by showing that the integer sorting algorithms, including PLIS and our algorithm, use $O(n\sqrt{\log r})$ work.
This explains why they are faster than comparison sort in practice, and asymptotically better in the range of $r=o(n^{\sqrt{\log n}})$.
Indeed, we show that we can achieve $O(\sqrt{\log r}\log n)$ span for unstable integer sort.
\textbf{To the best of our knowledge, this is the first practical parallel sorting algorithm that achieves $o(n\log n)$ work and $\polylog(n)$ span for a non-trivial setting of the integer key range $r=n^{O(1)}$.}\yan{Check if we want to claim this as a main contribution since it will need some justifications.}
We believe the theoretical contributions of this paper bridges the theory and practice of existing parallel sorting algorithms.
}














